Confidently Comparing Estimators with the c-value

Modern statistics provides an ever-expanding toolkit for estimating unknown parameters. Consequently, applied statisticians frequently face a difficult decision: retain a parameter estimate from a familiar method or replace it with an estimate from a newer or more complex one. While it is traditional to compare estimates using risk, such comparisons are rarely conclusive in realistic settings. In response, we propose the "c-value" as a measure of confidence that a new estimate achieves smaller loss than an old estimate on a given dataset. We show that it is unlikely that a large c-value coincides with a larger loss for the new estimate. Therefore, just as a small p-value supports rejecting a null hypothesis, a large c-value supports using a new estimate in place of the old. For a wide class of problems and estimates, we show how to compute a c-value by first constructing a data-dependent high-probability lower bound on the difference in loss. The c-value is frequentist in nature, but we show that it can provide validation of shrinkage estimates derived from Bayesian models in real data applications involving hierarchical models and Gaussian processes.

==> experiments.tex <==
\section{Application to Real Data}\label{sec:experiments}
Covid (smoothing \# cases) [Poisson noise]

%Weather (ncdc.noaa.gov/cdo-web/orders?id=2152957)\Cref{fig:logan_temperature}.
%\begin{figure}
%    \centering
%    \includegraphics[width=0.7\textwidth]{./figs/logan_temp_l=4_sigma=25.png}
%\caption{
%GP fit to weekly temperature at Logan airport in 2019.
%A squared exponential kernel was used with length-scale $l=4$ and signal variance $\sigma=25$ was used (chosen before looking at the data to reflect prior beliefs).
%The observation variance was as the average of the sample variances for each week across the years $2000-2019$.
%This provides a significant improvement $p=0.018$.}
%    \label{fig:logan_temperature}
%\end{figure}
%

